The Cpi-calculus: a Model for Confidential Name Passing

Sharing confidential information in distributed systems is a necessity in many applications, however, it opens the problem of controlling information sharing even among trusted parties. In this paper, we present a formal model in which dissemination of information is disabled at the level of the syntax in a direct way. We introduce a subcalculus of the pi-calculus in which channels are considered as confidential information. The only difference with respect to the pi-calculus is that channels once received cannot be forwarded later on. By means of examples, we give an initial idea of how some privacy notions already studied in the past, such as group creation and name hiding, can be represented without any additional language constructs. We also present an encoding of the (sum-free) pi-calculus in our calculus.

==> eptcsdata.tex <==
\providecommand{\firstpage}{115}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, A. Mavridou, A. Scalas (Eds.):\\
12th Interaction and Concurrency Experience (ICE 2019).\\
EPTCS 304, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.304.8}{10.4204/EPTCS.304.8}}

